Parameter-Based Value Functions

Traditional off-policy actor-critic Reinforcement Learning (RL) algorithms learn value functions of a single target policy. However, when value functions are updated to track the learned policy, they forget potentially useful information about old policies. We introduce a class of value functions called Parameter-Based Value Functions (PBVFs) whose inputs include the policy parameters. They can generalize across different policies. PBVFs can evaluate the performance of any policy given a state, a state-action pair, or a distribution over the RL agent's initial states. First we show how PBVFs yield novel off-policy policy gradient theorems. Then we derive off-policy actor-critic algorithms based on PBVFs trained by Monte Carlo or Temporal Difference methods. We show how learned PBVFs can zero-shot learn new policies that outperform any policy seen during training. Finally our algorithms are evaluated on a selection of discrete and continuous control tasks using shallow policies and deep neural networks. Their performance is comparable to state-of-the-art methods.

==> sections/method.tex <==
We augment the state and action-value functions, allowing them to receive as an input also the weights of a parametric policy.
The parameter-based state-value function (PSVF) $V(s, \theta) = {\ev}[R_t|s_t=s, \theta]$ is defined as the expected return for being in state $s$ and following policy parameterized by $\theta$. Similarly, the parameter-based action-value function (PAVF) $Q(s,a, \theta) = {\ev}[R_t|s_t=s, a_t=a, \theta]$ is defined as the expected return for being in state s, taking action $a$ and following policy parameterized by $\theta$.
In the off-policy setting, the objective to be maximized becomes:
\begin{equation*}
    J(\pi_{\theta^{*}})=\max_{\theta}\int_{\mathcal{S}} d^{\pi_b}(s) V(s, \theta) \de s = \max_{\theta}\int_{\mathcal{S}} \int_{\mathcal{A}} d^{\pi_b}(s)  \pi_{\theta}(a|s)  Q(s,a,\theta) \de a \de s.
\end{equation*}
The performance index $J$ can also be defined with respect to the start-value function~\citep{peters2008reinforcement}:
\begin{equation*}
    J_{\mu_0}(\pi_{\theta})=\int_{\mathcal{S}} \mu_0(s) V^{\pi}(s, \theta) \de s.
\end{equation*}
This notation allows us to omit the dependence on the state in the PSVF and learn a function $V(\theta)$ (named PVF) which is an approximation of $J_{\mu_0}(\pi_{\theta})$: \LK{I added $\mu_0$ here to the index}
\begin{equation*}
    V(\theta) := {\ev}_{s \sim \mu_0(s)}[V(s, \theta)] = \int_{\mathcal{S}} \mu_0(s) V(s, \theta) \de s = J_{\mu_0}(\pi_{\theta}).
\end{equation*}

